Bridge Girth: A Unifying Notion in Network Design

A classic 1993 paper by Alth\H{o}fer et al. proved a tight reduction from spanners, emulators, and distance oracles to the extremal function $\gamma$ of high-girth graphs. This paper initiated a large body of work in network design, in which problems are attacked by reduction to $\gamma$ or the analogous extremal function for other girth concepts. In this paper, we introduce and study a new girth concept that we call the bridge girth of path systems, and we show that it can be used to significantly expand and improve this web of connections between girth problems and network design. We prove two kinds of results: 1) We write the maximum possible size of an $n$-node, $p$-path system with bridge girth $>k$ as $\beta(n, p, k)$, and we write a certain variant for "ordered" path systems as $\beta^*(n, p, k)$. We identify several arguments in the literature that implicitly show upper or lower bounds on $\beta, \beta^*$, and we provide some polynomially improvements to these bounds. In particular, we construct a tight lower bound for $\beta(n, p, 2)$, and we polynomially improve the upper bounds for $\beta(n, p, 4)$ and $\beta^*(n, p, \infty)$. 2) We show that many state-of-the-art results in network design can be recovered or improved via black-box reductions to $\beta$ or $\beta^*$. Examples include bounds for distance/reachability preservers, exact hopsets, shortcut sets, the flow-cut gaps for directed multicut and sparsest cut, an integrality gap for directed Steiner forest. We believe that the concept of bridge girth can lead to a stronger and more organized map of the research area. Towards this, we leave many open problems, related to both bridge girth reductions and extremal bounds on the size of path systems with high bridge girth.

==> basedefs.tex <==

\section{Base Definitions and Results}

\subsection{Bridge-Free Path Systems}


% \begin{figure}
% \begin{center}
% \begin{tikzpicture}
% \draw [ultra thick, ->] (0, 0) -- (0, 12);
% \draw [ultra thick, ->] (0, 0) -- (12, 0);
% \node [align=center] at (-1.8, 6) {Function\\val};
% \node at (6, -1.5) {$p$};
% \node at (0, -0.5) {$1$};
% \node at (6, -0.5) {$n$};
% \node at (12, -0.5) {$n^2$};
% \node at (-0.5, 0) {$n$};
% \node at (-0.5, 6) {$n^{3/2}$};
% \node at (-0.5, 12) {$n^2$};

% %k=1
% \draw [thick, blue] (0, 0) -- (6, 12) node [midway, above, rotate=61] {$k=1$ (all)};

% %k=2
% \draw [thick, blue] (3, 0) -- (6, 6);
% \node [blue, rotate=60.5] at (3.2, 1.1) {$k=2$ ($\abeta, \abetastar$)};
% \draw [thick, blue] (2, 0) -- (6, 6);
% \node [blue, rotate=58] at (3.2, 2.4) {$k=2$ ($\beta, \betastar$)};

% \draw [thick, blue] (6, 6) -- (12, 12) node [midway, above, rotate=41] {$k=2$ (all)};
% \draw [fill=blue] (6, 6) circle [radius=0.15];

% %k=3
% \draw [thick, green] (3, 0) -- (12, 12) node [midway, green, above, rotate=55] {$k=3$ ($\beta, \abeta$ upper)};
% \draw [fill=blue] (6, 4) circle [radius=0.15];
% \draw [fill=blue] ({4/5*6}, 2.4) circle [radius=0.15];
% \draw [fill=blue] ({7/8*6}, 3) circle [radius=0.15];
% \draw [fill=blue] ({8/7*6}, {36/7}) circle [radius=0.15];
% \draw [fill=blue] ({5/4*6}, 6) circle [radius=0.15];

% \draw [ultra thick, red] (3, 0) to[bend right=15] (12, 12);

% \draw [red] (8, 3.5) -- (5, 1.6);
% \node [red, fill=white] at (9.5, 3.5) {$k=3$ (all lower)};

% %k=infty
% \draw [red, ultra thick] (4, 0) to[bend right=5] (9, 6.13);
% \node [red, rotate=51] at (5.9, 1.5) {$k=\infty$ (all lower)};
% \end{tikzpicture}
% \caption{Asymptotic bounds for functions, drawn to $\log n$ scale.  Blue lines are matching upper/lower bounds, green lines are upper bounds, red lines are lower bounds.  For visual clarity the lower bounds curves have been ``smoothed'' rather than drawn with piecewise accuracy.  Subpolynomial improvements in the $k=3$ upper bounds are not represented in this graph.}
% \end{center}
% \end{figure}

% \begin{table}
% \begin{center}
% \begin{tabular}{lll}
% \hline
% \textbf{Value of $k$} & \textbf{Relationship} & \textbf{Justification}\\
% \hline
% \multirow{5}{*}{all} & $\beta^* \ge \beta \ge \abeta$ and $\beta^* \ge \abeta^* \ge \abeta$ & Immediate from defs\\
% & $\beta(n, p) + \beta(n', p') \le \beta(n+n', p+p')$, same for other $\beta$ fn's & Disjoint union of LBs (immediate)\\
% & $\abeta(\ell n, \ell p) \ge \ell \cdot \beta(n, p)$ for $\ell := \frac{\beta(n, p)}{p}$ & \multirow{2}{*}{Theorem \ref{thm:layering}}\\
% & $\abetastar(\ell n, \ell p) \ge \ell \cdot \betastar(n, p)$ for $\ell := \frac{\betastar(n, p)}{p}$ &\\
% & {\color{red} any general relationship between $\beta, \betastar$ or $\abeta, \abetastar$?} & \color{red} open problem\\
% \hline
% \multirow{2}{*}{$3$} & $\abeta(n, p, 3) = \abeta(p, n, 3)$ & Corollary \ref{cor:abetathreedual}\\
% & {\color{red} Does $\abetastar(n, p) = \abetastar(p, n)$?} & {\color{red} open problem}\\
% \hline

% \multirow{5}{*}{$\infty$} & $\beta=\Theta\left(\abeta\right)$ & Corollary \ref{cor:inftyacyclic}\\
% & \color{red} Improve previous layering theorem with this technique? & \color{red} open problem\\
% & {\color{red} Does $\betastar = \Theta\left(\abetastar\right)$?} & {\color{red} open problem}\\
% & {\color{red} Does $\beta(n, p, \log n) = n^{o(1)} \cdot \beta(n, p, \infty)$?} & {\color{red} open problem}\\
% & {\color{red} shortcut sets seem to imply $\beta, \abetastar$ relationship -- what exactly?} & \color{red} open problem\\
% \hline
% \end{tabular}
% \caption{Reductions Among Functions}
% \end{center}
% \end{table}
% \gbnoteinline{killing this entire table since it all has to do with $\abeta$ lol}



==> beta4bound.tex <==
\input{preamble}

\title{$\beta(n, p, 4)$ upper bound notes}
\author{} 
%\author{Greg, Gary, Ohad \\ University of Michigan EECS}
\date{}

\begin{document}

\maketitle

\thispagestyle{empty}

\begin{abstract}
Scratch work here for $\beta(n, p, 4)$ upper bounds, hopefully eventually to be copied over to the main file.
\end{abstract}

\section{Proof}

We will prove:
\begin{theorem}
$\abeta(n, p, 4) = O(n^{3/5} p^{7/10} + n + p)$
\end{theorem}

Let $S = (V, \Pi)$ be an acyclic path system with bridge girth $>4$, $n$ nodes, and $p$ paths.
We assume without loss of generality\gbnote{cite this or something} that all paths have length exactly $\ell$ for some parameter $\ell$, and all nodes have degree $\Theta(d)$, where $d$ is the average degree of the system.
We assume that $\ell, d$ are both at least sufficiently large constants.
We note the identity $nd = p\ell$, which will be occasionally useful.

\subsection{Proof Setup and Overview}

Consider the following process, parametrized by some $1 \le h \le \ell$, that generates a random induced subsystem $S' \subseteq S$:
\begin{itemize}
\item Choose a path $\pi_b \in \Pi$ uniformly at random, called the \emph{base path}.
\item Let $Q \subseteq \Pi$ be the set of paths that intersect $\pi_b$, not including $\pi_b$ itself.
(Note that $|Q| = \Theta(\ell d)$.)
Let $V'$ be the set of nodes $v' \in V$ with the following property: there exists a node $u \in \pi_b$ and a path $q \in Q$ with $u \le v$ in $q$ and with $|q[u \leadsto v]| < h$.
(That is, $u, v$ are at least $0$ and at most $h-1$ positions apart in $q$.)

\item Define $S' = (V', \Pi')$ by taking the induced subsystem of $S$ on the vertex subset $V'$.
\end{itemize}

\begin{figure} [ht]
\begin{center}
    \begin{tikzpicture}
    \draw [fill=black] (0, 0) circle [radius=0.15];
    \draw [fill=black] (2, 0) circle [radius=0.15];
    \draw [fill=black] (4, 0) circle [radius=0.15];
    \draw [fill=black] (6, 0) circle [radius=0.15];
    \draw [ultra thick, ->] (-0.5, 0) -- (6.5, 0);
    \draw [ultra thick, ->] (-0.125, -0.5) -- (0.5, 2);
    \draw [ultra thick, ->] (0.125, -0.5) -- (-0.5, 2);
    
    \draw [ultra thick, ->] (1.875, -0.5) -- (2.5, 2);
    \draw [ultra thick, ->] (2.125, -0.5) -- (1.5, 2);
    
    \draw [ultra thick, ->] (3.875, -0.5) -- (4.5, 2);
    \draw [ultra thick, ->] (4.125, -0.5) -- (3.5, 2);
    
    \draw [ultra thick, ->] (5.875, -0.5) -- (6.5, 2);
    \draw [ultra thick, ->] (6.125, -0.5) -- (5.5, 2);
    
    \draw [decorate, decoration = {brace}] (-1, 0) --  (-1, 2);
    \node at (-2.5, 1) {$h$ nodes/path};
    \node at (7, 0) {$\pi_b$};
    
    \draw (0.3, 0) arc (0:180:0.3);
    
    \node at (-2.5, -0.5) {$\Theta(d)$ paths/node};
    \draw (-1.1, -0.5) -- (0, 0);
    
    \end{tikzpicture}
\end{center}
\caption{The random subsystem $S'$, generated with respect to ``height'' parameter $h$.}
\end{figure}

Note in the following that, since $S, S'$ are acyclic and $2$-bridge-free, any two paths intersect on at most one node.
We next make some structural observations on the intersection patterns exhibited by paths in $S$ (or in $S'$).
For an ordered pair of paths $(\pi_1, \pi_2) \in \Pi^2$, we define
$$R_S(\pi_1, \pi_2) := \left\{ r \in \Pi \ \mid \ (r \cap \pi_1) < (r \cap \pi_2) \in r \right\},$$
that is, $R_S(\pi_1, \pi_2)$ is the set of all paths that intersect a node in $\pi_1$ and then strictly later a node in $\pi_2$.
We will also use notation $R_{S'}(\pi_1, \pi_2)$, in which case the paths are drawn from the paths that survive in the subsystem $S'$.

We next claim that no two distinct paths $r_1, r_2 \in R_S(\pi_1, \pi_2)$ intersect $\pi_1$ at the same node, nor do they intersect $\pi_2$ at the same node; otherwise $r_1, r_2, \pi_2$ form a $3$-bridge (in the first case) or $r_1, r_2, \pi_1$ form a $3$-bridge (in the second case).
\begin{center}
    \begin{tikzpicture}
    \draw [ultra thick, ->] (0, 0) -- (0, 1.5);
    \draw [ultra thick, ->] (1, 0) -- (1, 1.5);
    \node at (0, -0.5) {$\pi_1$};
    \node at (1, -0.5) {$\pi_2$};
    
    \draw [fill=black] (0, 1) circle [radius=0.15];
    \draw [fill=black] (1, 1) circle [radius=0.15];
    \draw [fill=black] (1, 0.5) circle [radius=0.15];

    
    \draw [ultra thick, ->] (-0.5, 1) -- (1.5, 1);
    \draw [ultra thick, ->] (-0.5, 1.25) -- (1.5, 0.25);

    
    \node at (-1, 1) {$r_1$}; 
    \node at (-1, 1.5) {$r_2$}; 

    
    \node at (3, 0.5) {$3$-bridge};
    \end{tikzpicture}
\end{center}

Thus the paths in $R_S(\pi_1, \pi_2)$ intersect $\pi_1, \pi_2$ at distinct nodes.
The node ordering in $\pi_1$ induces an ordering of the paths $r \in R$ (by the order of the point $r \cap \pi_1$), and the node ordering in $\pi_2$ similarly induces another ordering of the paths in $R$.
Our next observation is that these orderings are the same.
In other words: for any two paths $r_1, r_2 \in R$, it is not possible to simultaneously have that
$$(r_1 \cap \pi_1) < (r_2 \cap \pi_1) \in \pi_1$$
and also that
$$(r_1 \cap \pi_1) > (r_2 \cap \pi_1) \in \pi_2.$$
The reason for this is that otherwise, $\pi_1, \pi_2, r_1, r_2$ form a $4$-bridge, with $r_1$ as the river.

\begin{center}
    \begin{tikzpicture}
    \draw [ultra thick, ->] (0, -0.5) -- (0, 1.5);
    \draw [ultra thick, ->] (1, -0.5) -- (1, 1.5);
    \draw [ultra thick, ->] (-0.5, -0.5) -- (1.5, 1.5);
    \node at (-1, -0.5) {$r_1$};
    \node at (0, -1) {$\pi_1$};
    \node at (1, -1) {$\pi_2$};
    \draw [fill=black] (0, 0) circle [radius=0.15];
    \draw [fill=black] (1, 0) circle [radius=0.15];
    
    \draw [fill=black] (0, 1) circle [radius=0.15];
    \draw [fill=black] (1, 1) circle [radius=0.15];
    
    \draw [ultra thick, ->] (-0.5, 1.5) -- (1.5, -0.5);
    
    \node at (-1, 1.5) {$r_2$}; 
    
    \node at (3, 0.5) {$4$-bridge};
    \end{tikzpicture}
\end{center}

To summarize: the paths in $R$ are arranged roughly as in the following picture, with their points of intersection with $\pi_1, \pi_2$ increasing along both paths.


\begin{center}
    \begin{tikzpicture}
    \draw [ultra thick, ->] (0, -0.5) -- (0, 2);
    \draw [ultra thick, ->] (1, -0.5) -- (1, 2);
    \draw [ultra thick, ->] (-0.5, 0) -- (1.5, 0);
    \node at (-1, 0) {$\pi_b$};
    \node at (0, -1) {$\pi_1$};
    \node at (1, -1) {$\pi_2$};
    \draw [fill=black] (0, 0) circle [radius=0.15];
    \draw [fill=black] (1, 0) circle [radius=0.15];
    
    \draw [fill=black] (0, 0.75) circle [radius=0.15];
    \draw [fill=black] (1, 1) circle [radius=0.15];

    \draw [fill=black] (0, 1.5) circle [radius=0.15];
    \draw [fill=black] (1, 1.5) circle [radius=0.15];
    
    \draw [ultra thick, ->] (-0.5, 0.625) -- (1.5, 1.125);
    \draw [ultra thick, ->] (-0.5, 1.5) -- (1.5, 1.5);
    
    \node at (-1, 0.625) {$r_1$};
    \node at (-1, 1.5) {$r_2$};

    \node at (3, 0.5) {Can happen};
    
    \end{tikzpicture}
\end{center}

Next, it will be helpful to \emph{charge} some node pairs in $S'$ to associated path pairs in $Q$.
For each ordered pair of distinct nodes $(x, y)$ with $x < y \in \pi'$ for some $\pi' \in \Pi'$, we notice by construction that there is a distinct pair of paths $(q_1, q_2) \in Q^2$ with $x \in q_1, y \in q_2$.
We charge $(x, y)$ to this pair $(q_1, q_2)$.
Note that the paths in $Q$ partition the nodes in $V'$, and so there is a unique way to charge each such pair $(x, y)$.

Our previous structural observations imply that we charge at most $h$ node pairs to each pair $(q_1, q_2) \in H$.
Additionally, we note that if $q_1 \cap \pi_b = q_2 \cap \pi_b$, then no pairs are charged to $(q_1, q_2)$, since this would imply a $3$-bridge.

\begin{center}
    \begin{tikzpicture}
    \draw [ultra thick, ->] (0, -0.5) -- (0, 2);
    \draw [ultra thick, ->] (-0.2, -0.3) -- (1.2, 1.8);
    \draw [ultra thick, dotted, ->] (-0.5, 0) -- (1.5, 0);
    \node at (-1, 0) {$\pi_b$};
    \node at (0, -1) {$q_1$};
    \node at (-0.4, -0.6) {$q_2$};
    \draw [fill=black] (0, 0) circle [radius=0.15];
    
    \draw [fill=black] (0, 1.5) circle [radius=0.15];
    \draw [fill=black] (1, 1.5) circle [radius=0.15];
    
    \draw [ultra thick, ->] (-0.5, 1.5) -- (1.5, 1.5);
    
    \node at (-1, 1.5) {$\pi$};

    \node at (3, 0.5) {$3$-bridge};
    
    \end{tikzpicture}
\end{center}


We can now show via straightforward counting that the maximum possible value of $\|S'\|_2^2$ is $O(\ell^2 d^2 h)$.
Note that this is \emph{not} our final bound on $\|S'\|_2^2$, it will be strictly improved in the rest of our argument.
Nonetheless, we will sketch the argument here, to build intuition for the strategy to follow.
We analyze the paths in $S'$ in three different categories.
\begin{itemize}
\item The paths $q \in Q$ have length $\le h$ each.
Thus, they contribute $|Q| \cdot h^2 = O(\ell d h^2) \le O(\ell^2 d h)$ to the value of $\|S'\|_2^2$, which is negligible.

\item Some paths $\pi' \in \Pi'$ might only contain one node.
Since there are $O(\ell d h)$ nodes in $V'$, and each node has degree $\Theta(d)$, in total these paths may contribute at most $O(\ell d^2 h)$ to the value of $\|S'\|_2^2$, which is negligible.

\item Finally, we consider the remaining paths $\pi' \in \Pi' \setminus Q$ that contain at least two nodes.
Each such path has $\Theta(|\pi'|^2)$ ordered node pairs $(x, y)$ where $x < y \in \pi'$.
Thus, it suffices to bound the number of ordered pairs of this type.
By our previous analysis, each such pair is charged to some $(q_1, q_2) \in Q^2$, and each pair in $Q^2$ is charged at most $h$ times, we count $|Q|^2 h = \Theta(\ell^2 d^2 h)$ node pairs of this type.
\end{itemize}

With this initial bound in place, we can now introduce a parameter of $S$ that will be the focus of our main argument.
We define the \emph{gap} of the original system $S$ as the quantity
$$g(h) := \mathbb{E}\left[ \frac{\|S'\|_2^2}{\ell^2 d^2 h} \right]$$
where the expectation is over the randomness in generating $S'$.
Intuitively, up to constants, the gap measures the expected fraction of this initial upper bound on $\|S'\|_2^2$ that is actually realized.
The maximum conceivable value is $g(h)=O(1)$, but it could also be polynomially sub-constant.
Our goal in the next to parts are to prove that:
\begin{itemize}
\item (Lemma \ref{lem:goodgapdep}) In the case where $g(h)$ is nontrivially small it implies an improved bound on the size of $S$, and

\item (Lemma \ref{lem:?}) We must in fact have that $g(h)$ is nontrivially small.
\end{itemize}

\subsection{Analysis Based on Gap}




Let
$$\mathcal{R}_S := \sum \limits_{(\pi_1, \pi_2) \in \Pi^2} \left| R_S(\pi_1, \pi_2) \right|.$$
The size of $\|S\|_2^2$ can be related to $\mathcal{R}_S$ as follows:
\begin{lemma} \label{lem:arrbound}
$\|S\|_2^2 = \Theta\left( \frac{ \mathcal{R}_S }{d^2} \right)$
\end{lemma}
\begin{proof}
Recall we have assumed that $\ell$ at least a large constant, and thus all paths in $\Pi$ have $\ge 2$ nodes.
As before, it thus suffices to only count node pairs of the form $x < y \in \pi$ for some path $\pi \in \Pi$.

For each such node pair $(x, y)$, there are $\Theta(d)$ paths in $\Pi$ that intersect $x$ and $\Theta(d)$ paths in $\Pi$ that intersect $y$.
Thus, this node pair $(x, y)$ causes us to add $\pi$ to $\Theta(d^2)$ different sets $R_S(\pi_1, \pi_2)$ with $(\pi_1, \pi_2) \in \Pi^2$.
So the pair $(x, y)$ contributes $\Theta(d)^2$ points to the value of $\mathcal{R}_S$.
It follows that $\|S\|_2^2 \cdot d^2 = \Theta(\mathcal{R}_S)$, and the lemma follows by rearranging. 
\end{proof}

Consider a fixed ordered pair of paths $(\pi_1, \pi_2) \in \Pi^2$.
Our next goal will be to prove a lower bound on the expected number of node pairs that are charged to the pair $(\pi_1, \pi_2)$ when we create $S'$.
That is: when we generate $S'$, if $\pi_1, \pi_2 \in Q$, then we may charge some node pairs $(x, y)$ to the pair $(\pi_1, \pi_2)$.
In the case where $\pi_1 \notin Q$ or $\pi_2 \notin Q$, then we charge $0$ node pairs to $(\pi_1, \pi_2)$.
Our goal is to bound the expected number of charges.
We prove:
\begin{lemma} \label{lem:paircharge}
For each $(\pi_1, \pi_2) \in \Pi^2$, the expected number of node pairs charged to $(\pi_1, \pi_2)$ is
$$\Omega\left(|R_S(\pi_1, \pi_2)|^2 \cdot \frac{h}{\ell p}\right).$$
\end{lemma}
\begin{proof}
For paths $r, r' \in R_S(\pi_1, \pi_2)$, let us say that $r'$ is \emph{close behind} $r$ if, letting
\begin{align*}
x &= r \cap \pi_1\\
y &= r \cap \pi_2\\
x' &= r' \cap \pi_1\\
y' &= r' \cap \pi_2,
\end{align*}
we have
$$0 \le |\pi_1[x \leadsto x']| < h \qquad \text{and} \qquad 0 \le |\pi_2[y \leadsto y']| < h.$$
(Thus, $r$ is considered to be close behind itself.)
Note that, if $r$ is selected as the base path in $S'$, then the number of node pairs charged to $(\pi_1, \pi_2)$ is exactly the number of paths in $R_S(\pi_1, \pi_2)$ that are close behind $r$.
Let us say that $r$ is \emph{typical} if there are at least
$$|R_S(\pi_1, \pi_2)| \cdot \frac{h}{4\ell p}$$
paths in $R_S(\pi_1, \pi_2)$ close behind.
We can lower bound the number of typical paths $r$ by counting them as follows.
Consider the paths $r \in R_S(\pi_1, \pi_2)$ in the order they intersect $\pi_1, \pi_2$, starting with the earliest points of intersection.
If $r$ is typical, add $1$ to the total.
Otherwise, if $r$ is not typical, then we skip the next $|R_S(\pi_1, \pi_2)| \cdot \frac{h}{4 \ell}$ paths in the ordering (including $r$; whether or not these paths are typical), and then we continue.
Each time we skip, since $r$ is atypical, the next path in the ordering progresses at least $h$ positions along $\pi_1$, or at least $h$ positions along $\pi_2$.
Since $|\pi_1| = |\pi_2| = \ell$, we can thus only skip $2h/\ell$ times.
It follows that only $\le |R_S(\pi_1, \pi_2)| /2$ paths get skipped.
Hence $\Omega(|R_S(\pi_1, \pi_2)|)$ paths are typical.

Each typical path in $R_S(\pi_1, \pi_2)$ is selected as the base path for $S'$ with probability $1/p$, and if selected, we charge $\Omega\left( |R_S(\pi_1, \pi_2)| \cdot h/(\ell p) \right)$ paths to $(\pi_1, \pi_2)$.
The lemma follows.
\end{proof}

\begin{lemma} \label{lem:arrsumbound}
$\mathbb{E}\left[ \| S' \|_2^2 \right] = \Omega\left(\frac{h}{\ell p^3} \cdot \mathcal{R}_S^2 \right)$
\end{lemma}
\begin{proof}
We can lower bound the expected value of $\|S'\|_2^2$ by counting the expected number of node pairs $(x, y)$ that are charged to some $(q_1, q_2) \in Q^2$.
By Lemma \ref{lem:paircharge}, this is
\begin{align*}
\mathbb{E}[\{|(x, y) \in V^2 \ \mid \ (x, y) \text{ charged} \}] &= \Omega\left(\sum \limits_{(\pi_1, \pi_2) \in \Pi^2} \left| R_S(\pi_1, \pi_2)\right|^2 \cdot \frac{h}{\ell p} \right)\\
&= \frac{h}{\ell p^3} \cdot \Omega\left(\sum \limits_{(\pi_1, \pi_2) \in \Pi^2} \left| R_S(\pi_1, \pi_2)\right|^2  \right) \cdot p^2\\
&=  \Omega\left(\frac{h}{\ell p^3} \cdot \left( \sum \limits_{(\pi_1, \pi_2) \in \Pi^2} \left| R_S(\pi_1, \pi_2)\right|\right)^2 \right) \tag*{Cauchy-Schwarz}\\
&=  \Omega\left(\frac{h}{\ell p^3} \cdot \mathcal{R}_S^2 \right). \tag*{\qedhere}\\
\end{align*}
\end{proof}

Using the previous two lemmas, we can now prove:
\begin{lemma} \label{lem:goodgapdep}
$\|S\| = O\left( n^{2/3} p^{2/3} g(h)^{1/3} \right)$.
\end{lemma}
\begin{proof}
We have
\begin{align*}
\|S\|_2^2 &= \Theta\left( d^{-2} \mathcal{R}_S \right) \tag*{Lemma \ref{lem:arrbound}}\\
&= d^{-2} \cdot O\left( \frac{\ell p^3}{h} \cdot \mathbb{E}\left[\|S'\|_2^2 \right] \right)^{1/2} \tag*{Lemma \ref{lem:arrsumbound}}\\
&= d^{-1} \cdot O\left( \ell^3 p^3 \cdot \frac{\mathbb{E}\left[\|S'\|_2^2 \right]}{\ell^2 d^2 h} \right)^{1/2} \\
&= d^{-1} \cdot O\left( \ell^3 p^3 \cdot g(h) \right)^{1/2} \\
&= O\left( \frac{\ell^{3/2} p^{3/2}}{d} \cdot g(h)^{1/2} \right)\\
&= O\left( n \ell^{1/2} p^{1/2} \cdot g(h)^{1/2} \right) \tag*{$nd=\ell p$}\\
&= O\left( n \|S\|^{1/2} \cdot g(h)^{1/2} \right) \tag*{$\ell p = \|S\|$.}
\end{align*}
Next, by Cauchy-Schwarz we have that $\|S\|^2 \le p\|S\|_2^2$, so we may continue
\begin{align*}
\frac{\|S\|^2}{p} \le &= O\left( n \|S\|^{1/2} \cdot g(h)^{1/2} \right)\\
\|S\|^{3/2} &= O\left( n p \cdot g(h)^{1/2} \right)\\
\|S\| &= O\left( n^{2/3} p^{2/3} g(h)^{1/3}\right). \tag*{\qedhere}
\end{align*}
\end{proof}

\subsection{Part 2: A Limit on Gap}

\begin{lemma}
For any possible realization of $S'$, if the average length of a path in $S'$ is at least $2$, then we have $\|S'\|_2^2 \le ???$
\end{lemma}

First we define some terms to help with this proof.
For a node $v \in V'$ let
$$N(v) := \{u \ne v \in V' \ \mid \ u, v \in \pi \text{ for some } \pi \in \Pi'\}.$$
We have:
\begin{lemma}
$\sum \limits_{v \in V'} |N(v)| = \Theta\left( \|S'\|_2^2 \right).$
\end{lemma}
\begin{proof}
Each path $\pi \in \Pi'$ contributes $|\pi|^2$ to the value of $\|S'\|_2^2$.
Additionally, for each node $u \in \pi$, it contributes $|\pi|-1$ to the value of $|N(u)|$, and hence $|\pi|(|\pi|-1)$ to the sum of $|N(v)|$ over all nodes.

Each path $\pi$ of length $|\pi| \ge 2$ thus contributes $\Theta(|\pi|^2)$ to both $\|S'\|_2^2$ and to the sum of $|N(v)|$ over all nodes.
Paths of length $|\pi|=1$ contribute $1$ to $\|S'\|_2^2$, and $0$ to the sum of $|N(v)|$ over all nodes.
However, since the average path length is at least $2$, the paths of length $1$ only increase $\|S'\|_2^2$ by a constant factor, which may be ignored.
\end{proof}


Now, let $v^* \in V'$ be a node sampled uniformly at random.
Say that a path $\pi \in \Pi$ is \emph{witnessed} if it intersects any node in $N(v)$.
We have:
\begin{lemma}
$$\mathbb{E}\left[\sum \limits_{\pi \in \Pi' \mid \pi \text{ witnessed}} |\pi| \right] = \frac{\sum \limits_{v \in V'} |N(v)|^2 }{n'}$$
\end{lemma}
\begin{proof}
Consider an arbitrary node $u$.
In the event that $u \in N(v^*)$, all paths intersecting $u$ are witnessed, and we will \emph{charge} their length to $u$.
Notice that no path may intersect two distinct nodes in $N(v^*)$, and so...

\gbnoteinline{pausing here: bad case is dominated nodes :(}

We include $u \in N(v^*)$ iff $v^* \in N(u)$, and hence
$$\Pr[u \in N(v^*)] = \frac{|N(u)|}{n'}.$$
If $u \in N(v^*)$, then the contribution of the paths through $u$ to the sum of witnessed path lengths is $\ge N(u)$.
Thus, the expected contribution of paths through $u$ to the sum of witnessed path lengths is at least
$$\frac{|N(u)|}{n'} \cdot N(u).$$
\end{proof}


$$\sum \limits_{q \in \Pi' \mid q \text{ witnessed}} |q| \le \sum \limits_{q \in \Pi'} |q| \le O\left(h \ell d^2 \right),$$
since there are $O(h \ell d)$ nodes in $S'$, each of degree $\Theta(d)$.
Meanwhile, in order to compute the expected sum of witnessed path lengths, we introduce a new term: for a node $v \in V'$, the \emph{adjusted degree} $\alpha(v)$ is
$$\alpha(v) := \sum \limits_{q \in Q | v \in q} |q|.$$
Notice that the probability of $v \in N(v)$ is exactly $\alpha(v)-1$, as any node may be sampled besides $v$ itself.


\subsection{lol i suck this is also scratch Part 2: Analysis Based on Path Counting}


We now introduce a separate parameter of $S$ that we will analyze.
Let
$$\psi(h) :=  \mathbb{E}\left[\frac{|\Pi'|}{p}\right],$$
that is, $\psi(h)$ is the expected fraction of paths from $S$ that survive (have at least one node) in $S'$.
Much like the previous section, the maximum conceivable value of $\psi(h)$ is $1$, and our goal is to prove a lemma that is meaningful in the case where $\psi(h)$ is significantly smaller.
We do so by relating $\psi(h)$ to the gap.
We remark that this proof will only use that $S'$ has bridge girth $>3$, i.e., the additional fact that $S'$ lacks $4$-bridges is not exploited in the following argument, which might signal room for improvement.

\begin{lemma}
$g(h) = O\left(\psi(h) \cdot \frac{p}{\ell d^2}\right).$
\end{lemma}
\begin{proof}
Consider a realization of $S' = (V', \Pi')$ and let $p'$ be the number of paths that survive.
Our first goal is to show that
$$\|S'\|_2^2 = O(\ell h p')$$
(deterministically), and then we will massage this expression slightly to prove the lemma.

Choose a node $v \in V'$ uniformly at random.
Let us say that a path $\pi \in \Pi'$ is \emph{witnessed} if there exists a path $q \in \Pi'$ with $v < (q \cap \pi) \in q$; that is, $q$ intersects $v$ and then later a node in $\pi$.
Our strategy is to lower bound the expected number of witnessed paths.
Consider an arbitrary path $q \in \Pi'$.
Our sampled node $v$ is contained in $q$ with probability $|q|/n'$, where $n'$ is the number of nodes in $V'$.
Conditional on the event $v \in q$, in expectation there are $\Theta(|q|)$ nodes following $v$ along $q$, and since all nodes have degree $\Theta(d)$, we thus witness $\Theta(|q|d)$ paths in expectation.

Moreover, we notice that no two paths $q_1, q_2 \in \Pi'$, with $v \in q_1 \cap q_2$, can cause the same path to be witnessed.
This is because if $\pi$ intersects both $q_1$ and $q_2$, then $\pi, q_1, q_2$ form a $3$-bridge.
We thus have:
\begin{align*}
p' \ge \mathbb{E}\left[\left|\{\pi \in \Pi' \ \mid \ \pi \text{ witnessed}\}\right|\right] &\ge \sum \limits_{q \in \Pi'} \Theta\left(\frac{|q|}{n'} \cdot |q|d\right)\\
&= \Theta\left(\frac{d}{n'} \sum \limits_{q \in \Pi'} |q|^2 \right)\\
&= \Theta\left(\frac{d}{n'} \|S'\|_2^2 \right)\\
&= \Omega\left(\frac{1}{\ell h} \cdot \|S'\|_2^2\right) \tag*{since $n' = O(\ell d h)$.}
\end{align*}
Rearranging, we get
$$\|S'\|_2^2 = O(\ell h p')$$
which was our initial bound.
We now continue:
\begin{align*}
\mathbb{E}\left[\|S'\|_2^2\right] &= \mathbb{E}\left[O(\ell h p')\right]\\
g(h) \cdot \ell^2 d^2 h &= O\left(\ell h p \cdot \psi(h)\right)\\
g(h) &= O\left(\psi(h) \cdot \frac{p}{\ell d^2}\right). \tag*{\qedhere}
\end{align*}
\end{proof}

\gbnoteinline{could continue to simplify from here, unclear if useful}



\subsection{scratcch for real}

We again use the random subsystem $S' = (V', \Pi')$, defined with respect to a parameter $h$, and let $p' := |\Pi'|$.

The maximum conceivable value of $\psi(h)$ is $p$.
Our goal here is to establish an upper bound on the expected size of $S'$ that benefits from the case where $\psi(h)$ is small.
\begin{lemma} \label{lem:sub3bound}
Letting $p'' := |\Pi''|$ be the number of paths that survive in $S''$, we have
$$\|S'\|_2^2 = O\left( \ell h \cdot p'' \right).$$
\end{lemma}
\begin{proof}

\begin{itemize}
\item long paths $q$ that witness long paths $\pi$,
\item short paths $q$ that witness long paths $\pi$,
\item long paths $q$ that witness short paths $\pi$, and
\item short paths $q$ that witness short paths $\pi$.
\end{itemize}

Our strategy is to argue that, in expectation, a constant fraction of the  paths

\emph{long-witnessed} if there exists $q \in \Pi''$ with $v < (q \cap \pi) \in q$ (that is, $q$ intersects $v$ and then later a node in $\pi$, and $q$ is a long enough path to survive in $\Pi''$).
We say that $\pi$ is \emph{short-witnessed}


\end{proof}

\subsection{Part 3: Gap vs.\ Path Counting}

Now we will consider four parameters: $g(h), g(\ell), \psi(h), \psi(\ell)$.
The previous two parts establish that, if \emph{any} of these parameters is nontrivially small, then we have a nontrivial upper bound on the size of $S$.
The last part of our proof is to show that these parameters cannot all be big at the same time.




\subsection{Case 2: ...(scratch? idk)}

[exposition]




\begin{lemma}
The expected number of paths in $S'$ is $\Omega\left( g(h) \cdot \ell d^2 \right)$.
\end{lemma}
\gbnoteinline{sloppy with expectations -- fix}
\begin{proof}
$S'$ has $O(\ell d h)$ nodes, and by definition of gap we have
$$\mathbb{E}\left[\|S'\|_2^2 \right] = g(h) \cdot \ell^2 d^2 h.$$
Plugging into Lemma \ref{lem:sub3bound}, letting $p'$ be the number of paths in $S'$, we have
\begin{align*}
g(h) \cdot \ell^2 d^2 h &= O\left(\frac{p' \ell d h}{d} \right)
\end{align*}
which rearranges to
\begin{align*}
p' = \Omega\left( g(h) \cdot \ell d^2 \right). \tag*{\qedhere}
\end{align*}
\end{proof}

\begin{lemma}
The expected number of paths in $S'$ is $...$
\end{lemma}
\begin{proof}
\gbnoteinline{super sketchy lol}
average path length in $h=\ell$ system: $\ell^2 d$ nodes, at most $p$ paths, so
$$\ge \frac{\ell^2 d^2}{p}.$$

expected average path length squared in $h$ system:
$g(h) \cdot \ell^2 d^2 h / p(h)$ ish
so basically $g(h) / p(h)$ cuts in half??
\end{proof}



Prove lemma: if $i_S(h) \gg h^2/L^2$ then a nontrivially small number of paths give the bulk of $\|S'\|_2^2$.
Use lemma bounding $\|S'\|_2^2$ on this, with a nontrivially small p parameter.  Problem: that lemma depends on d, which might shrink when we focus on these small paths. oh no.  i could maybe pay a log factor by considering telescoping length windows but this annoys me.  maybe i should target a "branching-counting" version?? 

\section{Scratch}

\subsection{Intermediate Lemma}

\begin{lemma}
$\abeta^{(2)}(n, p, 3) = O\left( pn/d \right)$
\end{lemma}
\begin{proof}
Let $S = (V, \Pi)$ have bridge girth $>4$.
Choose a node $v \in V$ uniformly at random.
Let $\Pi_v \subseteq \Pi$ be the paths that contain $v$, and let $N_v$ be the nodes that come after $v$ in any path in $\Pi_v$.
Each node $u \in N_v$ has degree $d$, and thus there are $d-1$ paths in $\Pi_u \setminus \Pi_v$.
Thus we have
$$p \ge \Omega\left(d |N_v|\right).$$
Additionally, we count
$$\mathbb{E}[|N_v|] = \sum \limits_{\pi \in \Pi} \frac{|\pi|}{n} \cdot \Theta(|\pi|) = \|S\|_2^2 /n.$$
Thus we have
$$pn/d \ge \|S\|_2^2.$$
\end{proof}

\gbnoteinline{can we remove the d? does pL/n or something suffice and then L can be averaged?? hmm}

\subsection{Overlap Bounding}

Let $h$ be a parameter.
We will focus on a subsystem generated as follows.
Choose a path $\pi_b \in \Pi$ uniformly at random, henceforth called the ``base path.''
Let $V'$ be the set of all nodes contained in $\pi_b$, or contained in a path $\pi'$ that branches with $\pi_b$ in one of the $h$ positions immediately following the intersected node $\pi' \cap \pi_b$.
Let $S' = S[V']$ be the induced subsystem on this vertex set.
We have $|V'|=\Theta(h\ell d)$ in expectation (henceforth assumed) and moreover every node in $S'$ has degree $\Theta(d)$.

\begin{lemma}
The average length of a path in $S'$ is $O(\sqrt{\ell h})$.
\end{lemma}
\begin{proof}
By the previous lemma, we thus have
$$\sum_{\pi \in \Pi} |\pi \cap V'| = O\left( \ell h p \right).$$
By averaging (say Cauchy-Schwarz) the average length of a path in $S'$ is $\sqrt{\ell h}$.
\end{proof}

\subsection{Gap Analysis}

I need to think this through but it's like a "typical" h-window has relatively few branches??

Maybe the take on the previous part is that a random h-window has like $L^2 d^2 h$ possible bridgers, but we only really witness $Lhp$ of them.  that's not clearly interesting :(

\subsection{the rest?}




We let $\diamond$ be the set of all minimal diamonds.
The \defemph{gap} of a minimal diamond is the max length over the left and right sides, $\pi_\ell[w \leadsto y]$ and $\pi_r[y \leadsto z]$.
The \defemph{average gap} $g$ of the system $S$ is the average gap over all minimal diamonds.
That is:
$$g := \sum \limits_{a \in \diamond} \frac{\text{gap}(a)}{|\diamond|}.$$
We count:
\begin{lemma} \label{lem:diamondbound}
$|\diamond| = O\left(p^2 L/g \right)$
\end{lemma}
\begin{proof}
Consider any two paths $\pi_{\ell}, \pi_r \in \Pi$ and let $\diamond_{\ell, r}$ be the minimal diamonds that use $\pi_{\ell}, \pi_r$ as their (left, right) paths.
Since $|\pi_{\ell}| = |\pi_r| = L$, we have
$$\sum \limits_{a \in \diamond_{\ell, r}} \text{gap}(a) = O(L).$$
Unioning over all possible choices of $\pi_{\ell}, \pi_r$, we get
$$\sum \limits_{a \in \diamond} \text{gap}(a) = O\left( p^2 L \right).$$
Dividing both sides by $|\diamond|$, we then have
$$g = O\left( \frac{p^2 L}{|\diamond|} \right),$$
and the lemma follows by rearranging.
\end{proof}

Our proof will be a counting argument over the minimal diamonds in the system, but for technical reasons it is helpful to restrict attention to only ``typical'' minimal diamonds (called ``shiny'' in the following), which we define next.
\begin{itemize}
    \item Say that a minimal diamond has \defemph{low gap} if its gap is $\le 2g$.
    \item We define a pair of paths $(\pi_b, \pi_t)$ to be \defemph{productive} if they act as the (bottom, top) pair for at least $|\diamond|/(4p^2)$ low gap minimal diamonds.
    \item We define a minimal diamond to be  \defemph{shiny} if it has low gap, and also its (bottom, top) pair of paths is productive.
\end{itemize}
We notice that a constant fraction of all minimal diamonds are indeed shiny:
\begin{lemma}
There are $\Omega(|\diamond|)$ shiny diamonds in $S$.
\end{lemma}
\begin{proof}
By Markov's inequality, at least $|\diamond|/2$ minimal diamonds have low gap.
By unioning, there are $\le p^2 \cdot |\diamond|/(4p^2) = |\diamond|/4$ low gap minimal diamonds whose (bottom, top) pair of paths is not productive.
Thus, there are $\ge |\diamond|/4$ low gap minimal diamonds whose (bottom, top) pair of paths is productive, and these diamonds are shiny.
\end{proof}

\subsection{Bounding $g$ via random subsystems}

Let $S' = (V', \Pi')$ be a subsystem of $S$ generated by the following random process.
First we define the vertex set $V'$.
Randomly sample a path $\pi^* \in \Pi$.
The vertex set is
$$V' := \left\{v \ \mid \ \text{there is } \pi' \in \Pi, u \in \pi^* \cap \pi' \text{ and a subpath } \pi'[u \leadsto v] \text{ of length } \le 2g \right\}.$$
In other words, we form $V'$ by taking all nodes on $\pi^*$, and also for all paths $\pi'$ that intersect $\pi^*$, we take the first $2g$ nodes along $\pi'$ following its point of intersection with $\pi^*$.

\begin{center}
    \begin{tikzpicture}
    \draw [fill=black] (0, 0) circle [radius=0.15];
    \draw [fill=black] (2, 0) circle [radius=0.15];
    \draw [fill=black] (4, 0) circle [radius=0.15];
    \draw [fill=black] (6, 0) circle [radius=0.15];
    \draw [ultra thick, ->] (-0.5, 0) -- (6.5, 0);
    \draw [ultra thick, ->] (-0.125, -0.5) -- (0.5, 2);
    \draw [ultra thick, ->] (0.125, -0.5) -- (-0.5, 2);
    
    \draw [ultra thick, ->] (1.875, -0.5) -- (2.5, 2);
    \draw [ultra thick, ->] (2.125, -0.5) -- (1.5, 2);
    
    \draw [ultra thick, ->] (3.875, -0.5) -- (4.5, 2);
    \draw [ultra thick, ->] (4.125, -0.5) -- (3.5, 2);
    
    \draw [ultra thick, ->] (5.875, -0.5) -- (6.5, 2);
    \draw [ultra thick, ->] (6.125, -0.5) -- (5.5, 2);
    
    \draw [decorate, decoration = {brace}] (-1, 0) --  (-1, 2);
    \node at (-2.5, 1) {$2g$ nodes/path};
    \node at (7, 0) {$\pi^*$};
    
    \end{tikzpicture}
\end{center}

The system $S'$ has $n' = O(\ell d g)$ nodes.
Its paths are:
$$\Pi' := \left\{\pi' \in \Pi \ \mid \ (\pi^*, \pi') \text{ are the (bottom, top) paths of at least one shiny diamond} \right\}.$$
We have:
\begin{lemma}
The number of paths in $S'$ is $p' = O\left( \frac{L g d^2 p}{|\diamond|^{1/2}} \right)$.
\end{lemma}
\begin{proof}
By productivity, we notice that each path $\pi^t$ that survives in $S'$ contributes $\Omega(|\diamond|/p^2)$ shiny diamonds to $S'$.
Thus, its length in $S'$ must be
$$\left|\pi^t \right| = \Omega\left(\frac{|\diamond|^{1/2}}{p}\right).$$
Since we have
$$\|S'\|_1 = O(d) \cdot O(L g d) = O\left(L g d^2\right),$$
we have
$$p' \cdot \Omega\left( \frac{|\diamond|^{1/2}}{p}\right) = O\left( L g d^2\right)$$
and so
$$p' = O\left( \frac{L g d^2 p}{|\diamond|^{1/2}}\right).$$
\end{proof}

\begin{lemma}
$\mathbb{E}\left[\|S'\|_2^2\right] = \Omega\left( \frac{|\diamond|}{p} \right)$
\end{lemma}
\begin{proof}
Each shiny diamond survives in $S'$ if and only if its bottom path is sampled as $\pi^*$, so we expect $\Omega(|\diamond|/p)$ shiny diamonds to survive in $S'$.
Each surviving shiny diamond corresponds to a pair of nodes in $S'$ that lie on the same path.
Since $\|S'\|_2^2$ counts the number of such \emph{ordered} pairs of nodes, the bound follows.
\end{proof}

\gbnoteinline{some concerns about this method working out, I think the details need to be handled more carefully.  putting this on pause for now.}
\gbnoteinline{construction barrier, below here is garbage}

\begin{lemma}
Let $a, b$ be constants such that $\|S'\|_2^2 = O\left(n'^a p'^b \right)$.\gbnote{do I have to worry about annoying degenerate $+n$ or $+p$ cases here? not sure}
Then ...?
\end{lemma}
\begin{proof}
\begin{align*}
    \frac{|\diamond|}{p} &= O(L d g)^a \cdot O\left( \frac{L g d^2 p}{|\diamond|^{1/2}}\right)^b\\
    |\diamond|^{1+b/2} &= O\left(  L^{a+b} d^{a + 2b} g^{a+b} p^{1+b} \right)\\
    \left(\frac{p^2 L}{g}\right)^{1+b/2} &= O\left(  L^{a+b} \left(\frac{pL}{n} \right)^{a + 2b} g^{a+b} p^{1+b} \right) \tag*{Lemma \ref{lem:diamondbound} and $nd = pL$}\\
    L^{1 - 2a - 5b/2} &= O\left( p^{a + 2b - 1} n^{-a - 2b} g^{1 + a + 3b/2}\right)\\
    (pL^2)^{1/2 - a - 5b/4} &= O\left( p^{3b/4 - 1/2} n^{-a - 2b} g^{1 + a + 3b/2}\right)\\
    (pL^2)^{1/2 - a - 5b/4} &= O\left( p^{3b/4 - 1/2} n^{-a - 2b} g^{1 + a + 3b/2}\right)\\
    \|S\|_2^{1 - 2a - 5b/2} &= O\left( p^{3b/4 - 1/2} n^{-a - 2b} g^{1 + a + 3b/2} \right)
\end{align*}

xxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\begin{align*}
    L^{a+b} d^{a + 2b} g^{a+b} p^{1+b} &= \Omega(p^2 L / g)^{1+b/2} \tag*{Lemma \ref{lem:diamondbound}}\\
    L^{a+b/2 - 1} d^{a + 2b} g^{1+a+3b/2} &= p\\
    L^{a+b/2 - 1} \left(\frac{pL}{n}\right)^{a + 2b} g^{1+a+3b/2} &= p \tag*{nd=pL}\\
    L^{2a+5b/2 - 1} g^{1+a+3b/2} &= p^{1-a-2b} n^{a+2b}\\
    (pL^2)^{a + 5b/4 - 1/2} g^{1+a+3b/2} &= p^{1/2-3b/4} n^{a+2b}\\
\end{align*}
\end{proof}




\gbnoteinline{this is ridiculously sloppy with the probabilistic details lol.  i'm sure it's fixable but at some point we need to make this precise. do not be like me}\
\ghnoteinline{If I understand correctly, the argument for top pairs is  as follows. Suppose that  $Omega(\ell^2d^2)$ pairs are top pairs. Then $\pi^*$ is the only path that passes through these pairs. There are $O(p^2)$ pairs of paths in the graph. Therefore, since the `average' path uniquely passes through $\Omega(\ell^2d^2)$ pairs, we can argue that $p \cdot \ell^2d^2 \leq O(p^2)$, which gives an improvement.  My only gripe with this is that its possible for a pair of paths to be a top pair but $\pi^*$ to not be the unique path intersecting that pair. (the intersection could happen outside of $S'$). But I think this issue can be addressed pretty straightforwardly.  }

There exists a possible setting of $S'$ has all of the above properties, so in the following we will assume $S'$ is one such system.
We have:
\begin{lemma}
The average length of a path in $S' = (V', \Pi')$ is
$$\ell' = \frac{\|S'\|_1}{|\Pi'|} = \Omega\left( \ell/g\right).$$
\end{lemma}
\begin{proof}
Informally: the sum of path lengths in $S'$ is $\ell d^2 g$, and the sum of squared path lengths is $\ell^2 d^2$.
It follows that a typical path contributes $\cdot \ell/g$ more to the quantity ``sum of squared path lengths'' than to the quantity ``sum of path lengths.''
This implies that average path length is $\ge \ell/g$.
Formally, the proof is going to be a straightforward application of Cauchy-Schwarz I think.
\end{proof}

\ghnoteinline{I think this argument is certainly true if you assume that all paths in $S'$ have approximately the average path length $\ell'$. However, I'm less certain it's true if paths have different lengths. My concern is that long paths can contribute disproportionately to $\|S'\|_2$ because their length is squared. Formally speaking, if $\ell_1, \ell_2, \dots, \ell_k$ are the lengths of the paths in $S'$, and the average of these lengths is $\ell'$, then we can argue by Jensen's inequality that $\sum_i \ell_i^2 \geq \sum_i (\ell')^2$, but the other direction is not necessarily true.   Using this fact, we obtain the result $\ell' = O(\ell / g)$.  (We can get the same bound using Cauchy-Schwarz.)  Right now I'm trying to understand what does this say/mean about the `bad' case in our analysis.  }
\gbnoteinline{you're right!  good catch.  this is a bug.  I'll think about what to do with this...}

\begin{lemma} [Gap Bound]
We have $g = \Omega\left(\ell^{1/3}\right)$.\gbnote{This is too weak because it uses the $\beta(n, p, 3)$ bound.  Better bound will come from recursing here maybe?}
\end{lemma}
\begin{proof}
The system $S'$ has size $\|S'\|_1 = \ell d^2 g$ and average path length $\Omega(\ell/g)$.
Thus it has $O(d^2 g^2)$ paths.
Applying the $O(n^{2/3} p^{2/3})$ size bound,\gbnote{this is inefficient! we can apply a recursive bound here} we get that
$$\ell d^2 g = O\left( (\ell d g)^{2/3} (d^2 g^2)^{2/3} \right).$$
Rearranging, we get 
$$\ell^{1/3}g = O\left( g^2\right)$$
and so
$$g = \Omega\left(\ell^{1/3}\right).$$
\end{proof}


\subsection{Phase 2: using the gap bound}

The gap bound implies that a typical pair of paths $(\pi_1, \pi_2)$ has only $O(\ell^{2/3})$ paths going between them (otherwise, by pigeonhole, the average minimal diamond created between these paths has small gap).
Each path acts as a connector between $\ell^2 d^2$ pairs of other paths.
This gives the inequality $p \ell^2 d^2 = O(p^2 \ell^{2/3})$.
Rearranging, we get
$$p \ell^{4/3} d^2 = O(p^2)$$
and so
$$p^{4/3} \ell^{4/3} n^2 d^2 = O(p^{7/3} n^2)$$
and so
$$\|S\|^{10/3} = O(p^{7/3} n^2)$$
and so
$$\|S\| = O(p^{7/10} n^{3/5}).$$
\end{document}

==> bnpfournotes.tex <==
\input{preamble}

\title{$\beta(n, p, 4)$ upper bound notes}
\author{} 
%\author{Greg, Gary, Ohad \\ University of Michigan EECS}
\date{}

\begin{document}

\maketitle

\thispagestyle{empty}

\begin{abstract}
Scratch work here for $\beta(n, p, 4)$ upper bounds, hopefully eventually to be copied over to the main file.
\end{abstract}

\section{Proof}

We will prove:
\begin{theorem}
$\beta(n, p, 4) = O(p^{?} n^{?} + n + p)$\gbnote{fill in once argument is complete}
\end{theorem}

Let $S = (V, \Pi)$ be a path system with bridge girth $>4$, $n$ nodes, and $p$ paths.
We assume without loss of generality that all paths have length exactly $L$ for some parameter $L$, and all nodes have degree $\Theta(d)$, where $d$ is the average degree of the graph.
We assume that $L, d$ are both at least sufficiently large constants.
We note the identity $nd = pL$, which will be occasionally useful.

\subsection{Diamonds}

We say that a \defemph{minimal diamond} is a tuple of four distinct paths $\pi_{\ell}, \pi_r, \pi_t, \pi_b \in \Pi$ (see Figure~\ref{Figs:diamond}), which are respectively called the \emph{left, right, top, bottom} path of the diamond, such that there are four distinct nodes $w, x, y, z \in V$ with:
\begin{itemize}
    \item $\pi_b$ intersects nodes $w, x$ in that order,
    \item $\pi_t$ intersects nodes $y, z$ in that order,
    \item $\pi_{\ell}$ intersects nodes $w, y$ in that order,
    \item $\pi_r$ intersects nodes $x, z$ in that order.
    \item (minimal) there is \textbf{not} a fifth path $\pi_m \in \Pi$ that intersects a node on the subpath $\pi_{\ell}[w \leadsto y]$ followed by a node on the subpath $\pi_r[x \leadsto z]$.
\end{itemize}



\begin{figure}[htbp]
  \begin{center}
    \includegraphics[width=1.5in]{diamond}
    \end{center}
    \caption{...}
    \label{Figs:diamond}
\end{figure}


%\begin{center}
%    \begin{tikzpicture}
%    \draw [fill=black] (0, 0) circle [radius=0.15];
%    \draw [fill=black] (0, 2) circle [radius=0.15];
%    \draw [fill=black] (1, 2) circle [radius=0.15];
%    \draw [fill=black] (1, 0) circle [radius=0.15];
%    \draw [ultra thick, ->] (0, -0.5) -- (0, 2.5);
%    \draw [ultra thick, ->] (1, -0.5) -- (1, 2.5);
%    \draw [ultra thick, ->] (-0.5, 0) -- (1.5, 0);
%    \draw [ultra thick, ->] (-0.5, 2) -- (1.5, 2);
%    \draw [ultra thick, dashed, red, ->] (-0.5, 1) -- (1.5, 1);
%    \node [red] at (0.5, 1) {\Huge \bf $\times$};
%    \draw [fill=red] (0, 1) circle [radius=0.15];
%    \draw [fill=red] (1, 1) circle [radius=0.15];
%    \end{tikzpicture}
%\end{center}

We let $\diamond$ be the set of all minimal diamonds.
The \defemph{gap} of a minimal diamond is the max length over the left and right sides, $\pi_\ell[w \leadsto y]$ and $\pi_r[y \leadsto z]$.
The \defemph{average gap} $g$ of the system $S$ is the average gap over all minimal diamonds.
That is:
$$g := \sum \limits_{a \in \diamond} \frac{\text{gap}(a)}{|\diamond|}.$$
We count:
\begin{lemma} \label{lem:diamondbound}
$|\diamond| = O\left(p^2 L/g \right)$
\end{lemma}
\begin{proof}
Consider any two paths $\pi_{\ell}, \pi_r \in \Pi$ and let $\diamond_{\ell, r}$ be the minimal diamonds that use $\pi_{\ell}, \pi_r$ as their (left, right) paths.
Since $|\pi_{\ell}| = |\pi_r| = L$, we have
$$\sum \limits_{a \in \diamond_{\ell, r}} \text{gap}(a) = O(L).$$
Unioning over all possible choices of $\pi_{\ell}, \pi_r$, we get
$$\sum \limits_{a \in \diamond} \text{gap}(a) = O\left( p^2 L \right).$$
Dividing both sides by $|\diamond|$, we then have
$$g = O\left( \frac{p^2 L}{|\diamond|} \right),$$
and the lemma follows by rearranging.
\end{proof}

Our proof will be a counting argument over the minimal diamonds in the system, but for technical reasons it is helpful to restrict attention to only ``typical'' minimal diamonds (called ``shiny'' in the following), which we define next.
\begin{itemize}
    \item Say that a minimal diamond has \defemph{low gap} if its gap is $\le 2g$.
    \item We define a pair of paths $(\pi_b, \pi_t)$ to be \defemph{productive} if they act as the (bottom, top) pair for at least $|\diamond|/(4p^2)$ low gap minimal diamonds.
    \item We define a minimal diamond to be  \defemph{shiny} if it has low gap, and also its (bottom, top) pair of paths is productive.
\end{itemize}
We notice that a constant fraction of all minimal diamonds are indeed shiny:
\begin{lemma}
There are $\Omega(|\diamond|)$ shiny diamonds in $S$.
\end{lemma}
\begin{proof}
By Markov's inequality, at least $|\diamond|/2$ minimal diamonds have low gap.
By unioning, there are $\le p^2 \cdot |\diamond|/(4p^2) = |\diamond|/4$ low gap minimal diamonds whose (bottom, top) pair of paths is not productive.
Thus, there are $\ge |\diamond|/4$ low gap minimal diamonds whose (bottom, top) pair of paths is productive, and these diamonds are shiny.
\end{proof}

\subsection{Bounding $g$ via random subsystems}

Let $S' = (V', \Pi')$ be a subsystem of $S$ generated by the following random process.
First we define the vertex set $V'$.
Randomly sample a path $\pi^* \in \Pi$.
The vertex set is
$$V' := \left\{v \ \mid \ \text{there is } \pi' \in \Pi, u \in \pi^* \cap \pi' \text{ and a subpath } \pi'[u \leadsto v] \text{ of length } \le 2g \right\}.$$
In other words, we form $V'$ by taking all nodes on $\pi^*$, and also for all paths $\pi'$ that intersect $\pi^*$, we take the first $2g$ nodes along $\pi'$ following its point of intersection with $\pi^*$.

\begin{center}
    \begin{tikzpicture}
    \draw [fill=black] (0, 0) circle [radius=0.15];
    \draw [fill=black] (2, 0) circle [radius=0.15];
    \draw [fill=black] (4, 0) circle [radius=0.15];
    \draw [fill=black] (6, 0) circle [radius=0.15];
    \draw [ultra thick, ->] (-0.5, 0) -- (6.5, 0);
    \draw [ultra thick, ->] (-0.125, -0.5) -- (0.5, 2);
    \draw [ultra thick, ->] (0.125, -0.5) -- (-0.5, 2);
    
    \draw [ultra thick, ->] (1.875, -0.5) -- (2.5, 2);
    \draw [ultra thick, ->] (2.125, -0.5) -- (1.5, 2);
    
    \draw [ultra thick, ->] (3.875, -0.5) -- (4.5, 2);
    \draw [ultra thick, ->] (4.125, -0.5) -- (3.5, 2);
    
    \draw [ultra thick, ->] (5.875, -0.5) -- (6.5, 2);
    \draw [ultra thick, ->] (6.125, -0.5) -- (5.5, 2);
    
    \draw [decorate, decoration = {brace}] (-1, 0) --  (-1, 2);
    \node at (-2.5, 1) {$2g$ nodes/path};
    \node at (7, 0) {$\pi^*$};
    
    \end{tikzpicture}
\end{center}

The system $S'$ has $n' = O(\ell d g)$ nodes.
Its paths are:
$$\Pi' := \left\{\pi' \in \Pi \ \mid \ (\pi^*, \pi') \text{ are the (bottom, top) paths of at least one shiny diamond} \right\}.$$
We have:
\begin{lemma}
The number of paths in $S'$ is $p' = O\left( \frac{L g d^2 p}{|\diamond|^{1/2}} \right)$.
\end{lemma}
\begin{proof}
By productivity, we notice that each path $\pi^t$ that survives in $S'$ contributes $\Omega(|\diamond|/p^2)$ shiny diamonds to $S'$.
Thus, its length in $S'$ must be
$$\left|\pi^t \right| = \Omega\left(\frac{|\diamond|^{1/2}}{p}\right).$$
Since we have
$$\|S'\|_1 = O(d) \cdot O(L g d) = O\left(L g d^2\right),$$
we have
$$p' \cdot \Omega\left( \frac{|\diamond|^{1/2}}{p}\right) = O\left( L g d^2\right)$$
and so
$$p' = O\left( \frac{L g d^2 p}{|\diamond|^{1/2}}\right).$$
\end{proof}

\begin{lemma}
$\mathbb{E}\left[\|S'\|_2^2\right] = \Omega\left( \frac{|\diamond|}{p} \right)$
\end{lemma}
\begin{proof}
Each shiny diamond survives in $S'$ if and only if its bottom path is sampled as $\pi^*$, so we expect $\Omega(|\diamond|/p)$ shiny diamonds to survive in $S'$.
Each surviving shiny diamond corresponds to a pair of nodes in $S'$ that lie on the same path.
Since $\|S'\|_2^2$ counts the number of such \emph{ordered} pairs of nodes, the bound follows.
\end{proof}

\gbnoteinline{some concerns about this method working out, I think the details need to be handled more carefully.  putting this on pause for now.}
\gbnoteinline{construction barrier, below here is garbage}

\begin{lemma}
Let $a, b$ be constants such that $\|S'\|_2^2 = O\left(n'^a p'^b \right)$.\gbnote{do I have to worry about annoying degenerate $+n$ or $+p$ cases here? not sure}
Then ...?
\end{lemma}
\begin{proof}
\begin{align*}
    \frac{|\diamond|}{p} &= O(L d g)^a \cdot O\left( \frac{L g d^2 p}{|\diamond|^{1/2}}\right)^b\\
    |\diamond|^{1+b/2} &= O\left(  L^{a+b} d^{a + 2b} g^{a+b} p^{1+b} \right)\\
    \left(\frac{p^2 L}{g}\right)^{1+b/2} &= O\left(  L^{a+b} \left(\frac{pL}{n} \right)^{a + 2b} g^{a+b} p^{1+b} \right) \tag*{Lemma \ref{lem:diamondbound} and $nd = pL$}\\
    L^{1 - 2a - 5b/2} &= O\left( p^{a + 2b - 1} n^{-a - 2b} g^{1 + a + 3b/2}\right)\\
    (pL^2)^{1/2 - a - 5b/4} &= O\left( p^{3b/4 - 1/2} n^{-a - 2b} g^{1 + a + 3b/2}\right)\\
    (pL^2)^{1/2 - a - 5b/4} &= O\left( p^{3b/4 - 1/2} n^{-a - 2b} g^{1 + a + 3b/2}\right)\\
    \|S\|_2^{1 - 2a - 5b/2} &= O\left( p^{3b/4 - 1/2} n^{-a - 2b} g^{1 + a + 3b/2} \right)
\end{align*}

xxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\begin{align*}
    L^{a+b} d^{a + 2b} g^{a+b} p^{1+b} &= \Omega(p^2 L / g)^{1+b/2} \tag*{Lemma \ref{lem:diamondbound}}\\
    L^{a+b/2 - 1} d^{a + 2b} g^{1+a+3b/2} &= p\\
    L^{a+b/2 - 1} \left(\frac{pL}{n}\right)^{a + 2b} g^{1+a+3b/2} &= p \tag*{nd=pL}\\
    L^{2a+5b/2 - 1} g^{1+a+3b/2} &= p^{1-a-2b} n^{a+2b}\\
    (pL^2)^{a + 5b/4 - 1/2} g^{1+a+3b/2} &= p^{1/2-3b/4} n^{a+2b}\\
\end{align*}
\end{proof}




\gbnoteinline{this is ridiculously sloppy with the probabilistic details lol.  i'm sure it's fixable but at some point we need to make this precise. do not be like me}\
\ghnoteinline{If I understand correctly, the argument for top pairs is  as follows. Suppose that  $Omega(\ell^2d^2)$ pairs are top pairs. Then $\pi^*$ is the only path that passes through these pairs. There are $O(p^2)$ pairs of paths in the graph. Therefore, since the `average' path uniquely passes through $\Omega(\ell^2d^2)$ pairs, we can argue that $p \cdot \ell^2d^2 \leq O(p^2)$, which gives an improvement.  My only gripe with this is that its possible for a pair of paths to be a top pair but $\pi^*$ to not be the unique path intersecting that pair. (the intersection could happen outside of $S'$). But I think this issue can be addressed pretty straightforwardly.  }

There exists a possible setting of $S'$ has all of the above properties, so in the following we will assume $S'$ is one such system.
We have:
\begin{lemma}
The average length of a path in $S' = (V', \Pi')$ is
$$\ell' = \frac{\|S'\|_1}{|\Pi'|} = \Omega\left( \ell/g\right).$$
\end{lemma}
\begin{proof}
Informally: the sum of path lengths in $S'$ is $\ell d^2 g$, and the sum of squared path lengths is $\ell^2 d^2$.
It follows that a typical path contributes $\cdot \ell/g$ more to the quantity ``sum of squared path lengths'' than to the quantity ``sum of path lengths.''
This implies that average path length is $\ge \ell/g$.
Formally, the proof is going to be a straightforward application of Cauchy-Schwarz I think.
\end{proof}

\ghnoteinline{I think this argument is certainly true if you assume that all paths in $S'$ have approximately the average path length $\ell'$. However, I'm less certain it's true if paths have different lengths. My concern is that long paths can contribute disproportionately to $\|S'\|_2$ because their length is squared. Formally speaking, if $\ell_1, \ell_2, \dots, \ell_k$ are the lengths of the paths in $S'$, and the average of these lengths is $\ell'$, then we can argue by Jensen's inequality that $\sum_i \ell_i^2 \geq \sum_i (\ell')^2$, but the other direction is not necessarily true.   Using this fact, we obtain the result $\ell' = O(\ell / g)$.  (We can get the same bound using Cauchy-Schwarz.)  Right now I'm trying to understand what does this say/mean about the `bad' case in our analysis.  }
\gbnoteinline{you're right!  good catch.  this is a bug.  I'll think about what to do with this...}

\begin{lemma} [Gap Bound]
We have $g = \Omega\left(\ell^{1/3}\right)$.\gbnote{This is too weak because it uses the $\beta(n, p, 3)$ bound.  Better bound will come from recursing here maybe?}
\end{lemma}
\begin{proof}
The system $S'$ has size $\|S'\|_1 = \ell d^2 g$ and average path length $\Omega(\ell/g)$.
Thus it has $O(d^2 g^2)$ paths.
Applying the $O(n^{2/3} p^{2/3})$ size bound,\gbnote{this is inefficient! we can apply a recursive bound here} we get that
$$\ell d^2 g = O\left( (\ell d g)^{2/3} (d^2 g^2)^{2/3} \right).$$
Rearranging, we get 
$$\ell^{1/3}g = O\left( g^2\right)$$
and so
$$g = \Omega\left(\ell^{1/3}\right).$$
\end{proof}


\subsection{Phase 2: using the gap bound}

The gap bound implies that a typical pair of paths $(\pi_1, \pi_2)$ has only $O(\ell^{2/3})$ paths going between them (otherwise, by pigeonhole, the average minimal diamond created between these paths has small gap).
Each path acts as a connector between $\ell^2 d^2$ pairs of other paths.
This gives the inequality $p \ell^2 d^2 = O(p^2 \ell^{2/3})$.
Rearranging, we get
$$p \ell^{4/3} d^2 = O(p^2)$$
and so
$$p^{4/3} \ell^{4/3} n^2 d^2 = O(p^{7/3} n^2)$$
and so
$$\|S\|^{10/3} = O(p^{7/3} n^2)$$
and so
$$\|S\| = O(p^{7/10} n^{3/5}).$$
\end{document}


==> preamble.tex <==
%moved preamble to main so that arxiv doesn't get mad at us
